A Deep-Learning-Aided Pipeline for Efficient Post-Silicon Tuning

In post-silicon validation, tuning is to find the values for the tuning knobs, potentially as a function of process parameters and/or known operating conditions. In this sense, an more efficient tuning requires identifying the most critical tuning knobs and process parameters in terms of a given figure-of-merit for a Device Under Test (DUT). This is often manually conducted by experienced experts. However, with increasingly complex chips, manual inspection on a large amount of raw variables has become more challenging. In this work, we leverage neural networks to efficiently select the most relevant variables and present a corresponding deep-learning-aided pipeline for efficient tuning.

==> fig/tikz_plot/adv_res.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={black!15},
xlabel={Candidate variables},
xmajorgrids,
xmin=-0.94, xmax=10.94,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10},
xticklabels={c1,c2,c3,c4,t1,t2,t3,t4,t5,t6,t7},
y grid style={black!15},
ylabel={Importance scores},
ymajorgrids,
ymin=0, ymax=0.5,
ytick={0, 0.2, 0.4},
yticklabels={0, 0.2, 0.4},
ytick style={color=black},
width=1.\textwidth,
height=0.3\textwidth
]
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:-0.4+0.1,0) rectangle (axis cs:0.4-0.1,0.00262367958202958);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:0.6+0.1,0) rectangle (axis cs:1.4-0.1,0.0077632968313992);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:1.6+0.1,0) rectangle (axis cs:2.4,0.00492275506258011);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:2.6+0.1,0) rectangle (axis cs:3.4-0.1,0.00197922065854073);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:3.6+0.1,0) rectangle (axis cs:4.4-0.1,0.093560092151165);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:4.6+0.1,0) rectangle (axis cs:5.4-0.1,0.448696315288544);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:5.6+0.1,0) rectangle (axis cs:6.4-0.1,0.280308187007904);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:6.6+0.1,0) rectangle (axis cs:7.4-0.1,0.036508958786726);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:7.6+0.1,0) rectangle (axis cs:8.4-0.1,0.0914768800139427);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:8.6+0.1,0) rectangle (axis cs:9.4-0.1,0.0216594431549311);
\draw[draw=none,fill=color0,fill opacity=0.65] (axis cs:9.6+0.1,0) rectangle (axis cs:10.4-0.1,0.0105011817067862);
%\draw (axis cs:0,0.00262367958202958) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(10)};
%\draw (axis cs:1,0.0077632968313992) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(8)};
%\draw (axis cs:2,0.00492275506258011) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(9)};
%\draw (axis cs:3,0.00197922065854073) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(11)};
%\draw (axis cs:4,0.093560092151165) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(3)};
%\draw (axis cs:5,0.448696315288544) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(1)};
%\draw (axis cs:6,0.280308187007904) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(2)};
%\draw (axis cs:7,0.036508958786726) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(5)};
%\draw (axis cs:8,0.0914768800139427) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(4)};
%\draw (axis cs:9,0.0216594431549311) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(6)};
%\draw (axis cs:10,0.0105011817067862) node[
%  scale=0.8,
%  anchor=south,
%  text=black,
%  rotate=0.0
%]{(7)};
\end{axis}

\end{tikzpicture}


==> fig/tikz_plot/time_vs_var.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={black!15},
xlabel={\# Candidate variables},
xmajorgrids,
xmin=-1.405, xmax=53.705,
xtick style={color=black},
xtick={1.1,3.2,6.4,12.8,25.6,51.2},
xticklabels={11,32,64,128,256,512},
y grid style={black!15},
ylabel={Time [sec.]},
ymajorgrids,
ymin=29.725, ymax=462.575,
ytick style={color=black},
width=1.\textwidth,
height=0.3\textwidth
]
\addplot [thick, color0, mark=star, mark size=3pt]
table {%
1.1 49.4
3.2 62.5
6.4 89.9
12.8 129.2
25.6 243.7
51.2 442.9
};
\end{axis}

\end{tikzpicture}

